Retrofitting Multilingual Sentence Embeddings with Abstract Meaning Representation

We introduce a new method to improve existing multilingual sentence embeddings with Abstract Meaning Representation (AMR). Compared with the original textual input, AMR is a structured semantic representation that presents the core concepts and relations in a sentence explicitly and unambiguously. It also helps reduce surface variations across different expressions and languages. Unlike most prior work that only evaluates the ability to measure semantic similarity, we present a thorough evaluation of existing multilingual sentence embeddings and our improved versions, which include a collection of five transfer tasks in different downstream applications. Experiment results show that retrofitting multilingual sentence embeddings with AMR leads to better state-of-the-art performance on both semantic textual similarity and transfer tasks. Our codebase and evaluation scripts can be found at \url{https://github.com/jcyk/MSE-AMR}.

==> BuccTatoeba.tex <==
%\paragraph{BUCC}
%Bitext mining aims to identify sentence pairs that are translations in two corpora in different languages. Following \cite{artetxe-schwenk-2019-margin}, we evaluate on the BUCC mining task \cite{zweigenbaum2018overview}. We use a score function based on cosine distance of sentence embeddings and pairs above a score threshold is classified as parallel. We report the F1 score. 
%\paragraph{Tatoeba}
%The multilingual STS and BUCC datasets only cover a small set of languages. \newcite{artetxe-schwenk-2019-massively} introduced a dataset for 112 different languages. For each language, it has up to 1,000 English-aligned sentence pairs. Evaluation is performed by checking for each sentence if the the most similar sentence in the other language is the aligned one. We use cosine similarity and compute the accuracy in both directions (English to the other language and back).

% \begin{table*}[t]
%     \centering
%     \small
%     \begin{tabular}{lccccccc}
%     \toprule
%       \tf{Model} & \tf{fr-en} & \tf{de-en} & \tf{ru-en} & \tf{zh-en} &  \tf{Avg.}\\
%           \midrule
%           mBERT & 47.21 & 44.09 & 38.04 & 37.41 & 41.69 \\
%           XLM-R & 5.69 &  4.90 & 23.07 & 15.70 & 12.34 \\
%           mUSE & 86.25 & 88.49 & 89.10 & 86.85 & 87.67 \\
%           LASER & 92.40 & 95.41 & 92.28 & 91.65 & 92.94 \\
%           LaBSE & 92.52 & 95.86 & 92.45 & 92.99 & 93.45 \\
%           paraphrase & 85.95 & 90.07 & 87.81 & 87.68 & 87.88 \\
%     \bottomrule
%     \end{tabular}

%     \caption{
%         BUCC results of different sentence embedding models .
%     }
%     \label{tab:bucc}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \small
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%       \tf{Model} & \tf{ar} & \tf{de} & \tf{tr} & \tf{es} & \tf{fr} & \tf{it} & \tf{nl} & \tf{ka} & \tf{sw} & \tf{tl} & \tf{tt} &  \tf{Avg.}\\
%           \midrule
%           mBERT & 17.80  & 59.60  & 27.80  & 52.40  & 50.80  & 45.70  & 53.20  & 17.02  &  9.74  &  8.70  & 15.30 & 32.55 \\
%           XLM-R & 9.10  & 41.80  & 11.50  & 35.50  & 26.30  & 19.90  & 42.10  & 10.32  &  3.33  &  4.40  &  1.60  & 18.71 \\
%           mUSE & 79.50  & 98.20  & 93.60  & 94.60  & 93.60  & 94.20  & 93.90  &  3.08  & 14.10  & 16.10  & 15.60  & 63.32 \\
%           LASER & 91.40  & 99.10  & 97.80  & 97.80  & 95.50  & 95.40  & 96.70  & 39.68  & 53.59  & 53.00  & 28.10  & 77.10 \\
%           LaBSE & 90.60  & 99.30  & 98.20  & 98.10  & 96.10  & 95.30  & 97.50  & 95.71  & 89.49  & 98.00  & 87.30  & 95.05 \\
%           paraphrase & 95.60  & 99.00  & 98.20  & 98.60  & 96.20  & 96.50  & 97.70  & 97.32  & 21.54  & 20.00  & 19.20  & 76.35 \\
%     \bottomrule
%     \end{tabular}

%     \caption{
%         Tatoeba en$\Rightarrow$x results of different sentence embedding models .
%     }
%     \label{tab:Tatoeba1}
% \end{table*}

% \subsubsection{Transfer Tasks}
% zero-shot: mBERT$<$paraphrase$<$XLM-R$<$mUSE$<$LASER$<$LaBSE

% \begin{table*}[t]
%     \centering
%     \small
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%       \tf{Model} & \tf{ar} & \tf{de} & \tf{tr} & \tf{es} & \tf{fr} & \tf{it} & \tf{nl} & \tf{ka} & \tf{sw} & \tf{tl} & \tf{tt} &  \tf{Avg.}\\
%           \midrule
%           mBERT & 23.40  & 65.90  & 32.40  & 62.90  & 60.30  & 55.80  & 56.30  & 20.78  &  6.67  & 11.30  & 15.00  & 37.34 \\
%           XLM-R & 11.40  & 57.40  & 24.20  & 37.20  & 35.30  & 31.30  & 48.30  & 15.82  &  4.87  &  9.10  &  0.90  & 25.07 \\
%           mUSE & 82.40  & 98.10  & 94.40  & 96.30  & 93.30  & 94.50  & 94.00  &  2.14  & 13.33  & 16.40  & 15.80  & 63.70\\
%           LASER & 92.00  & 98.80  & 97.30  & 97.60  & 94.30  & 95.10  & 96.00  & 32.04  & 60.77  & 48.40  & 34.60  & 76.99 \\
%           LaBSE & 91.10  & 99.40  & 98.50  & 98.80  & 96.00  & 94.00  & 97.00  & 96.11  & 87.44  & 96.90  & 88.50  & 94.89 \\
%           paraphrase & 94.20  & 98.70  & 97.90  & 98.60  & 95.20  & 95.80  & 97.50  & 96.78  & 20.00  & 20.60  & 16.60  & 75.63 \\
%     \bottomrule
%     \end{tabular}

%     \caption{
%         Tatoeba x$\Rightarrow$en results of different sentence embedding models .
%     }
%     \label{tab:Tatoeba2}
% \end{table*}
